FactKG: Fact Verification via Reasoning on Knowledge Graphs

In real world applications, knowledge graphs (KG) are widely used in various domains (e.g. medical applications and dialogue agents). However, for fact verification, KGs have not been adequately utilized as a knowledge source. KGs can be a valuable knowledge source in fact verification due to their reliability and broad applicability. A KG consists of nodes and edges which makes it clear how concepts are linked together, allowing machines to reason over chains of topics. However, there are many challenges in understanding how these machine-readable concepts map to information in text. To enable the community to better use KGs, we introduce a new dataset, FactKG: Fact Verification via Reasoning on Knowledge Graphs. It consists of 108k natural language claims with five types of reasoning: One-hop, Conjunction, Existence, Multi-hop, and Negation. Furthermore, FactKG contains various linguistic patterns, including colloquial style claims as well as written style claims to increase practicality. Lastly, we develop a baseline approach and analyze FactKG over these reasoning types. We believe FactKG can advance both reliability and practicality in KG-based fact verification.

==> contents/4datacons_backup.tex <==
\textsc{FactKG} is constructed based on 2020 WebNLG, which is a resource that contains 45,040 pairs of RDF-triples from DBpedia and the corresponding texts. 
In our construction process, \textbf{mutation} methods found in FEVER are adopted, including \textit{Substitution} (Section~\ref{sec:ref}), \textit{Generalization} (Multi-hop claims in Section~\ref{sec:sup},~\ref{sec:ref}), \textit{Negation} (Section~\ref{sec:neg}), and \textit{Paraphrase} (Section~\ref{sec:coll}).
% In existing crowdsourced data~\citep{thorne2018fever}, lexical bias was strong when generating claims~\citep{schuster-etal-2019-towards, park2021faviq}. 
% % The mutated claims in \textsc{FactKB} are generated automatically, so it can be inferred that they contain less lexical bias.
% The automated generation of mutated claims in \textsc{FactKB} may lead to diminished lexical bias.
Especially, our paraphrasing strategy aims to alter the sentence to a colloquial style, rather than simply adjusting its syntactic structure. 

\subsection{Claim Generation}
\label{sec:gen}
% We use claim $C$, corresponding graph $G$, and $E$ is defined as the set of entities in $G$,  
% $Type (e)$ is defined as the set of types of entity $e$ in DBpedia.
After investigating all claims in two crowdsourced datasets, FEVER and FEVEROUS, we found that 99.7\% of the claims consist of a single sentence. Thus, we extracted single sentences from WebNLG based on the fact that people typically consider one claim to be a single sentence. A detailed algorithm for extracting single sentences is described in Appendix \ref{app:extract}.
\subsubsection{Supported Claims}
\label{sec:sup}

\textbf{One-hop}\hspace{5mm} 
 The extracted claims are utilized as one-hop single and multiple claims. Unique types of graphs are shown in Figure ??.\footnote{Some sentences contain more than 4 entities, but they were not included in claims due to their unnatural nature.} Four unique types of graphs are identified, and 26,879 basic claims are included. 

\textbf{Multi-hop}\hspace{5mm} 
Basically, multi-hop claim $C_M$ is generated by replacing the entity $e$ of one-hop claim $C$ with its type $t$. 
% Careful selection of both the entity $e$ in $C$ and its type $t$ is crucial. 
The entity $e$ is selected from the green nodes in Figure ??, but in graph type 4, either one or both of the two nodes are selected. Then, the type $t$ of the entity $e$ is extracted from DBpedia. However, each entity $e$ in DBpedia has several types $Types(e)$, so it is necessary to select one of them. 
To this end, calculate the perplexity scores of sentences that are replaced entity $e$ of $C$ with $e~(t_k)$ for all types $t_k \in Types (e)$ using GPT2-large~\citep{radford2019language}. A multi-hop claim is completely generated by replacing $e$ with the type $t_m$ that has the lowest perplexity. The generation of multi-hop claims can facilitate sentence generalization through the substitution of entities with their type words.

\textbf{Relation Existence}\hspace{5mm} 
A claim is formulated by extracting only the \{Head, Relation\} or \{Tail, Relation\} from the triple. However, it is possible that claims lacking meaningful content may be generated in this manner. For example, \textit{``Meyer Werft had a location.''} or \textit{``Papenburg is a location.''} can be generated from the triple (Meyer Werft, location, Papenbug). Thus, out of 522 relations in triples of one-hop claims, we extracted 22 relations that are considered to be meaningful. Claims are generated based on templates using these relations. There are two types of templates: \textit{i)} Head-Relation with 2 templates for 17 relations and \textit{ii)} Tail-Relation with a template for 5 relations. Templates used for both types and examples of generated claims are in the Appendix \ref{app:relx}.

\subsubsection{Refuted Claims}
\label{sec:ref}
Refuted claims are basically created by substituting some parts of supported claims in two ways. 

\textbf{Entity Substitution}\hspace{5mm}
We substitute an entity in the supported claim with another entity to create a refuted claim. In order to make a more natural claim, we replace the entity with another entity belonging to the same category. We obtain the entity set $E_C$, which has the same category as the entity $e_i$ to be replaced in claim $C$ (details in the Appendix \ref{app:entset}). Refuted claim $\tilde{C}$ is generated by randomly selecting an entity $e_j$ from the set $E_C$ and replacing $e_i$ with $e_j$ in claim $C$. To ensure that $\tilde{C}$ is refuted, we choose entity $e_j$ that satisfies the following two conditions. First, to select the entity $e_j$ that is not directly related to entities in $C$, $e_j$ is selected outside 4-hops from all entity nodes in $C$ on DBpedia. Second, we use a natural language inference (NLI) model, RoBERTa-base~\citep{DBLP:journals/corr/abs-1907-11692} trained on the MNLI dataset~\citep{N18-1101}, to conduct bidirectional NLI between the original and substituted claim. We choose  $e_j$ where both NLI($C$, $\tilde{C}$) and NLI($\tilde{C}$, $C$) are \textsc{Contradiction}\footnote{The notation NLI(\textit{p}, \textit{h}) represents the result of NLI when \textit{p} is assigned as the premise and \textit{h} as the hypothesis.}.

\textbf{Relation Substitution}\hspace{5mm}
We also substitute a relation in the supported claim with another relation to generate a refuted claim. Unlike entities, relations do not appear in sentences in their raw form. For example, the triple (Meyer Werft, location, Papenburg) can be expressed as \textit{``Meyer Werft is in Papenburg.''} or \textit{``Meyer Werft is located in Papenburg.''}. Thus, the meaning of the relation is preserved by substituting all entities without altering the structure of the sentence. For graph type 1, we extract sentences in which both entities appear as they are. Then, we replace the head and tail entities of a relation with a new pair of entities with the same type from another relation. The example claim is in Figure ??.

\subsubsection{Negation}
\label{sec:neg}
A negative expression is added to the claim to make it more realistic and challenging. The Relation Existence claims are created using the negative version of templates (in Appendix \ref{app:relx}), and One-hop and Multi-hop claims in Section \ref{sec:sup}and~\ref{sec:ref} for graph type 1 and 2 are used.

\textbf{Type 1}\hspace{5mm}
We use the Negative Claim Generation Model~\citep{lee2021crossaug} which was fine-tuned on the opposite claim set in WikiFactCheck-English dataset. In order to ensure the quality of the generated sentences, we oversample 100 sentences and only use those that contain negative expressions (e.g. `not' or `never') and preserve all entities. Also, similar to Entity Substitution in Section~\ref{sec:ref}, we only use sentences that NLI result with original sentences becomes \textsc{Contradiction} in bidirectional ways. When a negative expression is added, the label of the generated claim is reversed from the original claim.

\textbf{Type 2}\hspace{5mm}
It differs from type 1 in that there are two relations, allowing for the inclusion of negative expressions in two places. We employ the pretrained language model GPT-J 6B~\citep{gpt-j} to attach negative expressions to the first or/and second relation of the claim. We construct an in-context example set consisting of 16 claims, each with negative expressions attached to the first or/and second relation. The generated claims are then labeled differently based on whether they are one-hop or multi-hop. \textit{i)} One-hop claims: When a negative expression is added to supported claims, all of the claims become refuted. However, when it is added to refuted claims, the label depends on the position of the negative expression. In cases where the triple containing the substituted entity includes a negative expression, the label is designated as \textsc{Supported}. Conversely, other cases preserve the label \textsc{Refuted}. \textit{ii)} Multi-hop claims: Claims are labeled by the existence of an entity that meets the conditions included in the claim. For example, the Negation claim \textit{``AIDAstella was built by a company, not in Papenburg.''} is \textsc{Supported} if $x$ exists where the triples (AIDAstella, ShipBuilder, $x$) and ($x$, location, $y$) are in DBpedia and $y$ is not \textit{Papenburg}.
A more detailed labeling strategy is in Appendix ??.

% However, as each one-hop claim is based on one triple, the label depends on whether each triple has a negative expression. 


\subsection{Colloquial Style Transfer}
\label{sec:coll}
Rather than simply paraphrasing claims, we transform them into a colloquial style to make them more useful. Colloquial style transfer is performed using both model-based and the concept of presupposition. 

\subsubsection{Model based}
Motivated by \cite{kim-etal-2021-robust}, we construct a similar colloquial style transfer pipeline. Using this pipeline, all of the claims generated in Section \ref{sec:gen} are used as inputs, and colloquial-style claims are produced.

% First, we train FLAN T5-large~\cite{https://doi.org/10.48550/arxiv.2210.11416} to generate dialogue response given the grounding knowledge from Wizard of Wikipedia~\cite{dinan2019wizard}. 
We train FLAN T5-large~\cite{https://doi.org/10.48550/arxiv.2210.11416} to generate a dialogue response given the corresponding knowledge sentence from Wizard of Wikipedia~\cite{dinan2019wizard} to transform the sentence style from written language to spoken language. However, since the generated sentence may not retain all of the contents of the original claim or have a colloquial style, it is necessary to utilize an additional filing process.

First of all, to make more diverse samples using the model, we set the temperature to 20.0 and generate 500 samples with beam search. Among the 500 samples, only sentences with an edit distance of 6 or more from the original sentence are selected to prevent copy-paste. Then, only those that have verbs and the named entities are all preserved are retained\footnote{NLTK~\cite{bird2009natural} POS tagger and Stanza~\cite{qi2020stanza} NER module are used.}. Lastly, we use bidirectional NLI to preserve the original semantics. The generated sentences are retained when NLI ($O$, $G$) is \textsc{Entailment} and NLI ($G$, $O$) is not \textsc{Contradiction} where $O$ refers to the original sentence and $G$ refers to the generated sentence. On average, only 41.2 generated sentences were retained out of 500 samples, and for 34.0\% of the original sentences, no generated sentences remained. Following the filtering process, the AFLITE method \cite{sakaguchi2019winogrande}, which utilizes adversarial filtering, is applied to select the most colloquial style sentence among the surviving sentences.


% Then, we utilize the named entity recognition (NER) module from Stanza~\cite{qi2020stanza} to preserve named entities. Only samples in which all named entities of the original sentence are preserved survive. 

\subsubsection{Presupposition}
A presupposition is something the speaker assumes to be the case prior to making an utterance~\cite{yule1996pragmatics}. The part of the speaker's statement that is assumed to be true or false is considered as a claim in this study, and its veracity is evaluated.
There are several types of presuppositions, but for the purpose of our work, we have focused on three types that are clearly indicative of intent: Factive, Non-Factive, and Structural presuppositions.

\textbf{Factive Presupposition}\hspace{5mm} 
This is the assumption that something is true by the presence of some verbs such as “remember” and “realize”. If someone says “I remembered that Biden was Vice President.”, then it assumes that Biden was Vice President. We organize 8 templates to make factive presupposition claims, and the details are in Appendix \ref{app:factpre}.

\textbf{Non Factive Presupposition}\hspace{5mm}Unlike a factive presupposition, the assumption refers to something that is not true. For example, a speaker says ``I imagined that the Eiffel Tower was in America.'' when the Eiffel Tower was not in America. Claims that invert the label of the original sentences are created using this presupposition. We organize 3 templates to make claims, and the details are in Appendix \ref{app:nonfactpre}.

\textbf{Structural Presupposition}\hspace{5mm} 
This type is in the form of a question that presumes certain facts. We treat the question itself as a claim. For instance, When was Messi in Barcelona? assumes Messi was in Barcelona. 
% It is notable that this approach can be used as a criterion to determine unanswerable questions~\cite{kim2021linguist}. 
To create a natural sentence form, only claims corresponding to the existence of a relation and graph type 1 are constructed. The templates used are available in the Appendix \ref{app:structpre}. 

\subsection{Quality Control}

To evaluate the quality of our dataset, the labeling strategy and the output of the colloquial style transfer model are assessed.

\textbf{Labeling Strategy}\hspace{5mm} When a claim is made in the manner described in Section \ref{sec:sup}, the labeling of the claim is unproblematic as all supported claims have precise evidence graphs.
However, random substitution was used to generate the refuted claims, and as a result, the generated statement can be supported (e.g. \textit{``The White House is in Washington, D.C.''} to \textit{``The White House is America.''}). To assess this method, randomly sampled 1,000 substituted claims were reviewed by 2 graduate students. As a consequence, there was only one claim in which both participants identified as \textsc{Supported}, and there were five claims in which only one of them identified as \textsc{Supported}.

\textbf{Colloquial Style Transfer Model}\hspace{5mm} In order to evaluate the quality of the generated sentences, a survey was conducted that targeted colloquial style claims in the test set. Upon review by three graduate students, it was found that the proportion of claims resulting in a \textit{Loss of important information}, as selected by at least two out of the three reviewers, was ~~\%. To ensure the quality of the test set, only claims that received a rating of \textit{1) All facts are preserved} from at least two of the 3 reviewers were included in the test set. Survey details are in Appendix \ref{app:survey}. 

% Despite being generated by oversampling and subjected to multiple filtering steps, it cannot be guaranteed that every element of the original sentence is retained in the final outcome. 

\subsection{Data Split}
All triples are separated into three triple sets with a proportion of 8:1:1 (train, valid, test) and no overlap is ensured among them. To prevent the possibility of claims in the test set being inferred from knowledge acquired from the train data without graph evidence, the dataset is divided by the triple sets. 

==> tables/4datastat.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\begin{tabular}{c|cc|cccc|c}
\Xhline{1.5pt} 
\multirow{3}{*}{\textbf{Type}} & \multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Written}}} & \multicolumn{4}{c|}{\textbf{Colloquial style}}                                                                     & \multirow{3}{*}{\textbf{Total}} \\ \cline{4-7}
                      & \multicolumn{2}{c|}{}                         & \multicolumn{2}{c|}{\textbf{Model}}                                    & \multicolumn{2}{c|}{\textbf{Presupposition}}      &                        \\ \cline{2-7}
                      & \multicolumn{1}{c|}{\textbf{Supported}}    & \textbf{Refuted}   & \multicolumn{1}{c|}{\textbf{Supported}} & \multicolumn{1}{c|}{\textbf{\textbf{Refuted}}} & \multicolumn{1}{c|}{\textbf{Supported}} & \textbf{Refuted} &                        \\ \hline
one-hop               & \multicolumn{1}{c|}{942}          & 1074      & \multicolumn{1}{c|}{8904}      & \multicolumn{1}{c|}{7030}    & \multicolumn{1}{c|}{760}       & 820     & 19,530                 \\ \hline
conjuction            & \multicolumn{1}{c|}{8879}         & 11708     & \multicolumn{1}{c|}{7605}      & \multicolumn{1}{c|}{8303}    & \multicolumn{1}{c|}{307}       & 295     & 37,097                 \\ \hline
existence             & \multicolumn{1}{c|}{142}          & 138       & \multicolumn{1}{c|}{2028}      & \multicolumn{1}{c|}{2032}    & \multicolumn{1}{c|}{2422}      & 2410    & 9,172                  \\ \hline
multi-hop             & \multicolumn{1}{c|}{4655}         & 5584      & \multicolumn{1}{c|}{9262}      & \multicolumn{1}{c|}{7158}    & \multicolumn{1}{c|}{303}       & 300     & 27,262                 \\ \hline
negation              & \multicolumn{1}{c|}{424}          & 916       & \multicolumn{1}{c|}{5957}      & \multicolumn{1}{c|}{6509}    & \multicolumn{1}{c|}{957}       & 850     & 15,613                 \\ \hline
total                 & \multicolumn{2}{c|}{34,462}                   & \multicolumn{2}{c|}{64,788}                                   & \multicolumn{2}{c|}{9,424}               & 108,674                \\ \Xhline{1.5pt} 
\end{tabular}
\end{table*}

==> tables/exp_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\centering
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l|ccccc|c}
\Xhline{1.5pt}
\textbf{Model} & \textbf{One-hop}  & \textbf{Conjunction} & \textbf{Existence} & \textbf{Multi-hop} & \textbf{Negation} & \textbf{Total} \\ \hline
\textit{claim only} &  &  &  &  &  &  \\
\ \ BERT & 69.64  & 63.31 & 61.84 & 70.06 & 63.62 & 65.20 \\ 
\ \ BlueBERT & 60.03  & 60.15 & 59.89 & 57.79 & 58.90 & 59.93 \\
\ \ Flan-T5 & 62.17  & 69.66 & 55.29 & 60.67 & 55.02 & 62.70 \\
% RoBERTa & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
\hline
\textit{with evidence} &  &  &  &  &  &  \\
\ \ GEAR & 83.23  & 77.68 & 81.61 & 68.84 & 79.41 & 77.65 \\ \Xhline{1.5pt}
\end{tabular}%
}
\caption{The performance of baseline models on \textsc{FACTKG} datasets.
% \label{tab:results}
}
\end{table*}

==> tables/transfer_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|cc}
\Xhline{1.5pt}
\textbf{Model} & \textbf{Written $\rightarrow$ Spoken} & \textbf{Spoken $\rightarrow$ Written} \\ \hline
\textit{claim only} &  &  \\
\ \ BERT &  63.85&  69.43\\
\ \ BlueBERT &  56.28&  63.92\\
% \ \ Flan-T5 &  58.80&  69.02\\ 
\hline
\textit{with evidence} &  &  \\
\ \ GEAR &  75.43 & 78.80 \\ \Xhline{1.5pt}
\end{tabular}%
}
\caption{Experimental results.
\label{tab:transresults}
}
\end{table}
